See More, Detect Less? Taming Information Leakage in Multi-View Anomaly Detection

In multi-view anomaly detection, more cross-view information can actually hurt. When multiple inspection views are naively fused in a reconstruction-based pipeline, normal cues from intact views propagate to the decoder, which faithfully reconstructs anomalous regions, collapsing the reconstruction gap the detector depends on. We call this failure mode \emph{cross-view information leakage} and show that effective multi-view fusion must explicitly restrict the information reaching the decoder. Building on this insight, we present GLAD(Global-Local Attention Driven framework), the first framework combining vision foundation model features with local and global cross-view fusion for multi-view anomaly detection. The Multi-view Merging Attention (MMA) module performs local cross-view fusion at linear complexity with learnable view importance weighting and token-wise gating, letting each view selectively incorporate fine-grained evidence from other views at $\mathcal{O}(N)$ cost. The Object-Guided Attention (OGA) module captures global context by aggregating class tokens from all views into a single object-level representation and broadcasting it back to patch tokens via temperature-scaled sigmoid gating, replacing the original patch representations rather than adding a residual to preserve the reconstruction gap. Experiments on Real-IAD and MANTA-Tiny show that GLAD outperforms state-of-the-art methods across sample-, image-, and pixel-level metrics, confirming that principled information restriction is key to multi-view anomaly reasoning.

==> preamble.tex <==
\usepackage[dvipsnames]{xcolor,colortbl}         % colors
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{comment}

\RequirePackage{amsmath}
\let\Bbbk\relax
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage{bm} 
\RequirePackage{url}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{natbib}
\setcitestyle{square,comma,numbers,sort&compress}
\usepackage{graphicx}
\usepackage{caption,lipsum}
\usepackage{mathtools}
\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{booktabs} % For professional-looking tables
\usepackage{threeparttable} % For managing table footnotes

\definecolor{OursColor}{HTML}{F2F3F4}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{subcaption}

% Command
\newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\ul}[1]{{\underline{#1}}}


\righthyphenmin=4
\lefthyphenmin=4
\emergencystretch=1em

% Comment shortcuts
% --- Shawn
% \newcommand{\SC}[1]{\textcolor{blue}{\textbf{SC: #1}}}
% --- KP
\newcommand{\KP}[1]{\textcolor{teal}{\textbf{KP: #1}}}
% --- ours
\newcommand{\ourso}{\texttt{GLAD} (ours)\xspace}
\newcommand{\ours}{\texttt{GLAD}\@\xspace}

\newcommand{\etal}{\textit{et al.}}
\newcommand{\ie}{\textit{i.e.}\ }
\newcommand{\etc}{\textit{etc.}\ }


% Show the differences of rebuttal version.
\newcommand{\submission}{}

\ifx \submission \undefined
\definecolor{DarkGreen}{rgb}{0.00, 0.40, 0.00}
\definecolor{Red}{rgb}{1.0, 0.0, 0.0}
\newcommand{\wu}[1]{\textcolor{DarkGreen}{#1}}
\newcommand{\rb}[1]{\textcolor{Red}{#1}} % rebuttal
\newcommand{\SC}[1]{\textcolor{blue}{#1}}
\else
\newcommand{\wu}[1]{{#1}}
\newcommand{\rb}[1]{{#1}}
\newcommand{\SC}[1]{{#1}}
\fi


\def\gG{{\mathcal{G}}}

% Check-mark, Cross-mark
\usepackage{pifont}
\newcommand{\xmark}{\ding{55}}
\definecolor{checkmark}{HTML}{305AFF}
\definecolor{xmark}{HTML}{E62020}
\newcommand{\ccheck}{{\textcolor{checkmark}{\large\checkmark}}}
\newcommand{\ccross}{{\textcolor{xmark}{\large\xmark}}}


